Latent Space Representation for Shape Analysis and Learning

We propose a novel shape representation useful for analyzing and processing shape collections, as well for a variety of learning and inference tasks. Unlike most approaches that capture variability in a collection by using a template model or a base shape, we show that it is possible to construct a full shape representation by using the latent space induced by a functional map net- work, allowing us to represent shapes in the context of a collection without the bias induced by selecting a template shape. Key to our construction is a novel analysis of latent functional spaces, which shows that after proper regularization they can be endowed with a natural geometric structure, giving rise to a well-defined, stable and fully informative shape representation. We demonstrate the utility of our representation in shape analysis tasks, such as highlighting the most distorted shape parts in a collection or separating variability modes between shape classes. We further exploit our representation in learning applications by showing how it can naturally be used within deep learning and convolutional neural networks for shape classi cation or reconstruction, signi cantly outperforming existing point-based techniques.

==> sec-conclusion.tex <==
%!TEX root = main.tex
\section{Conclusions}
\label{sec:concl}

We have presented a novel latent representation for 3D shapes, in the context of a collection of related shapes. Our descriptors are based on functional maps networks connecting the shapes is the collection and are derived using the machinery of shape differences and adjoint functional maps.  They have many appealing properties, including invariance to rigid motions (and also to isometric ones, if desired) as well as full informativeness that permits reconstruction. We have demonstrated their use in extracting and highlighting variability of interest in a set of shapes, while also suppressing other variability that we regard as nuisance (and which may in fact manifest in larger geometric deformations). We believe that this highly nuanced understanding of shape distortions and variability is important for many applications in engineering, biology, and medicine.

The matrix form of our descriptor makes it suitable for input to learning algorithms and the use of convolutional neural networks. We have provided examples of such networks for both shape regression and shape reconstruction, with state-of-the-art results. We also note that the matrix nature of our latent code makes it a different mathematical object from the usual latent codes used in machine learning that are invariably points in high-dimensional Euclidean spaces. While with points we are quite limited to the operations we can do at the level of the latent representation (basically interpolations and vector-based analogies), our difference matrices reflect the internal structure of the shape better and may allow further structure-aware operations directly in the latent representation.

 
